Efficient fully dynamic elimination forests with applications to detecting long paths and cycles

We present a data structure that in a dynamic graph of treedepth at most $d$, which is modified over time by edge insertions and deletions, maintains an optimum-height elimination forest. The data structure achieves worst-case update time $2^{{\cal O}(d^2)}$, which matches the best known parameter dependency in the running time of a static fpt algorithm for computing the treedepth of a graph. This improves a result of Dvo\v{r}\'ak et al. [ESA 2014], who for the same problem achieved update time $f(d)$ for some non-elementary (i.e. tower-exponential) function $f$. As a by-product, we improve known upper bounds on the sizes of minimal obstructions for having treedepth $d$ from doubly-exponential in $d$ to $d^{{\cal O}(d)}$. As applications, we design new fully dynamic parameterized data structures for detecting long paths and cycles in general graphs. More precisely, for a fixed parameter $k$ and a dynamic graph $G$, modified over time by edge insertions and deletions, our data structures maintain answers to the following queries: - Does $G$ contain a simple path on $k$ vertices? - Does $G$ contain a simple cycle on at least $k$ vertices? In the first case, the data structure achieves amortized update time $2^{{\cal O}(k^2)}$. In the second case, the amortized update time is $2^{{\cal O}(k^4)} + {\cal O}(k \log n)$. In both cases we assume access to a dictionary on the edges of $G$.

==> figures/tikz-hypergraph.tex <==
% Needs
% \usetikzlibrary{calc}
% \usepackage{ifthen}

\def\rotateclockwise#1{
  % Rotate input point by 90 degrees clockwise.
  \newdimen\xrw
  \pgfextractx{\xrw}{#1}
  \newdimen\yrw
  \pgfextracty{\yrw}{#1}
  % \pgfpoint{-\y}{\x}
  \pgfpoint{\yrw}{-\xrw}
}

\def\rotatecounterclockwise#1{
  % Rotate input point by 90 degrees clockwise.
  \newdimen\xrcw
  \pgfextractx{\xrcw}{#1}
  \newdimen\yrcw
  \pgfextracty{\yrcw}{#1}
  % \pgfpoint{-\y}{\x}
  \pgfpoint{-\yrcw}{\xrcw}
}

\def\outsidespacerpgfclockwise#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Compute a length-radius vector perpendicular (clockwise)
  % to the vector from start point to end point.
  \pgfpointscale{#3}{
    \rotateclockwise{
      \pgfpointnormalised{
        \pgfpointdiff{#1}{#2}}}}
}

\def\outsidespacerpgfcounterclockwise#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Compute a length-radius vector perpendicular (counterclockwise)
  % to the line from start point to end point.
  \pgfpointscale{#3}{
    \rotatecounterclockwise{
      \pgfpointnormalised{
        \pgfpointdiff{#1}{#2}}}}
}

\def\outsidepgfclockwise#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Add to end point a length-radius vector perpendicular
  % (counter-clockwise) to the line from start point to end point.
  \pgfpointadd{#2}{\outsidespacerpgfclockwise{#1}{#2}{#3}}
}

\def\outsidepgfcounterclockwise#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Add to end point a length-radius vector perpendicular
  % (counter-clockwise) to the line from start point to end point.
  \pgfpointadd{#2}{\outsidespacerpgfcounterclockwise{#1}{#2}{#3}}
}

\def\outside#1#2#3{
  ($ (#2) ! #3 ! -90 : (#1) $)
}

\def\cornerpgf#1#2#3#4{
  % #1 = previous pgf point 
  % #2 = current pgf point
  % #3 = next pgf point
  % #4 = radius
  % Computes a path comprising a rounded corner on the outside of the angle #1#2#3.
  \pgfextra{
    \pgfmathanglebetweenpoints{#2}{\outsidepgfcounterclockwise{#1}{#2}{#4}}
    \let\anglea\pgfmathresult
    \let\startangle\pgfmathresult

    \pgfmathanglebetweenpoints{#2}{\outsidepgfclockwise{#3}{#2}{#4}}
    \pgfmathparse{\pgfmathresult - \anglea}
    \pgfmathroundto{\pgfmathresult}
    \let\arcangle\pgfmathresult
    \ifthenelse{180=\arcangle \or 180<\arcangle}{
      \pgfmathparse{-360 + \arcangle}}{
      \pgfmathparse{\arcangle}}
    \let\deltaangle\pgfmathresult

    \newdimen\x
    \pgfextractx{\x}{\outsidepgfcounterclockwise{#1}{#2}{#4}}
    \newdimen\y
    \pgfextracty{\y}{\outsidepgfcounterclockwise{#1}{#2}{#4}}
  }
  -- (\x,\y) arc [start angle=\startangle, delta angle=\deltaangle, radius=#4]
}

\def\corner#1#2#3#4{
  \cornerpgf{\pgfpointanchor{#1}{center}}{\pgfpointanchor{#2}{center}}{\pgfpointanchor{#3}{center}}{#4}
}

\def\hedgeiii#1#2#3#4{
  % #1#2#3 = tikz points
  % #4 = radius
  % Computes a path comprising the line of the points outside of the
  % convex hull H of the points #1#2#3 that have distance #4 to H.
  % Points #1#2#3 need to be in clockwise order.
  \outside{#1}{#2}{#4} \corner{#1}{#2}{#3}{#4} \corner{#2}{#3}{#1}{#4} \corner{#3}{#1}{#2}{#4} -- cycle
}

\def\hedgem#1#2#3#4{
  % #1#2 = tikz points
  % #3 = list of tikz points
  % #4 = radius
  % Computes a path comprising the line of the points outside of the convex hull H of the points #1#2[#3] that have distance #4 to H.
  % Points #1#2[#3] need to be vertices of a convex polygon and in clockwise order.
  
  \outside{#1}{#2}{#4}
  \pgfextra{
    \def\hgnodea{#1}
    \def\hgnodeb{#2}
  }
  foreach \c in {#3} {
    \corner{\hgnodea}{\hgnodeb}{\c}{#4}
    \pgfextra{
      \global\let\hgnodea\hgnodeb
      \global\let\hgnodeb\c
    }
  }
  \corner{\hgnodea}{\hgnodeb}{#1}{#4}
  \corner{\hgnodeb}{#1}{#2}{#4}
  -- cycle
}

\def\hedgeii#1#2#3{
  % #1#2 = tikz points
  % #3 = radius
  \hedgem{#1}{#2}{}{#3}
}

\def\hedgei#1#2{
  % #1 = tikz point
  % #2 = radius
  (#1) circle [radius = #2]
}

==> intro.tex <==
\section{Introduction}\label{sec:intro}

\noindent The \textbf{\boldmath$k$-path} problem is probably one of the most intensively studied problems of parameterized complexity: 
given a graph $G$ (directed or undirected, depending on the variant) and an integer $k$, decide whether $G$ contains a simple path on $k$ vertices (not necessarily induced).
The first fixed-parameter algorithm for $k$-path (both directed and undirected) was given by Monien~\cite{Monien85} as early as in 1985.
This algorithm runs in time $\Oh(k!\cdot nm)$ and is an elegant example of the use of {\em{representative sets}}, 
which by now became an important part of the parameterized complexity toolbox, see~\cite[Chapter~12]{platypus}.

Next, Bodlaender~\cite{Bodlaender93} proposed an algorithm with running time $\Oh(k!\cdot 2^k\cdot n)$, however working only for the undirected variant of the problem.
The idea is to construct a depth-first-search (DFS) forest~$F$ of the graph. 
If $F$ has depth at least $k$ then it immediately uncovers a $k$-path. 
Otherwise, $F$ can be turned into
a tree decomposition of width at most $k$, on which a dynamic programming algorithm running in time $\Oh(k!\cdot 2^k\cdot n)$ can be employed.
Thus, Bodlaender's approach~\cite{Bodlaender93} was precursive for contemporary decomposition techniques that are widespread in parameterized complexity; see~\cite[Chapter~7]{platypus}.

Later, $k$-path was again in the spotlight due to the work of Alon et al.~\cite{AlonYZ95}, who introduced the {\em{color-coding}} technique in order to give a randomized $(2e)^k\cdot n^{\Oh(1)}$-time algorithm for 
the problem, both in the undirected and the directed variant. This algorithm can 
be derandomized within time complexity $2^{\Oh(k)}\cdot n^{\Oh(1)}$, and in fact 
it was the first algorithm that achieved a single-exponential parametric factor
of the form $2^{\Oh(k)}$. The technique of color-coding turned out to be widely applicable in many other settings and became one of the most fundamental tools in the design of parameterized algorithms;
see~\cite[Chapter~5]{platypus}.

Finally, the search for efficient algorithms for $k$-path was pivotal in the development of algebraic techniques in parameterized complexity. 
Koutis~\cite{Koutis08} and Williams~\cite{Williams09} gave randomized algorithms for directed $k$-path with running times $2^{3k/2}\cdot n^{\Oh(1)}$ and $2^{k}\cdot n^{\Oh(1)}$, respectively;
see also~\cite{BjorklundHKK17} for a more modern presentation.
These developments laid foundations for {\em{algebraic coding}} and {\em{monomial testing}}, which by now are the core algebraic techniques of parameterized complexity; see~\cite[Chapter~10]{platypus}.
While for undirected $k$-path, Bj\"orklund~\cite{Bjorklund14} improved the running time to $1.66^k\cdot n^{\Oh(1)}$, the question whether there is a $c^k\cdot n^{\Oh(1)}$-time algorithm for directed $k$-path for any $c<2$ remains one of the most tantalizing open questions in the area.

\paragraph*{Dynamic \boldmath$k$-path.}
As witnessed by the discussion above, the $k$-path problem has served as the main protagonist in the development of several fundamental directions in parameterized complexity.
In this work we are interested in another view, namely that of {\em{dynamic algorithms}}.
Consider the following setting. 
We are given a graph $G$ whose vertex set remains invariant, but the edge set is modified over time by insertions and deletions.
We wish to always be able to answer the following query: does $G$ contain a simple path on $k$ vertices?
The goal is to develop a data structure that maintains this answer using as little time per update as possible, where the complexity is measured both in terms of $n$ and $k$.

This question was first investigated by Alman et al.~\cite{AlmanMW17}, who presented a data structure working for the undirected variant 
that uses $k!\cdot 2^{\Oh(k)}\cdot \mathsf{DC}(n)$ time per update and $2^{\Oh(k)}\cdot \log n$ time per query, 
where $\mathsf{DC}(n)$ denotes the query/update time for a data structure maintaining dynamic connectivity. In general, there are several possibilities for an implementation of dynamic connectivity, 
yet they all achieve an update time that is polylogarithmic in $n$; see the discussion in~\cite{AlmanMW17}. The data structure of Alman et al.~\cite{AlmanMW17} is based on dynamization of the standard color-coding approach.
Thus, the polylogarithmic factors --- originating both from dynamic connectivity and from color-coding --- seem hard to avoid.
We remark that, for the directed variant of the problem, Alman et al.~\cite{AlmanMW17} showed that under plausible assumptions from fine-grained complexity, any dynamic data structure needs update time 
$\Omega(n^\delta)$ for some $\delta>0$, already for $k=5$. This shows a qualitative difference between the directed and the undirected variants in the dynamic setting.
%\todo[inline]{Y: I don't understand how this sentence is compatible with the next sentence and our result. Doesn't it say that we need to depend on~$n$ in the update time?\\ MiPi: The lower bound is for directed variant,
%our result is for the undirected variant. I added some text to make it clearer.}

This raises a question: is there a data structure for the dynamic undirected $k$-path problem that would offer update time depending only on $k$, without any factors polylogarithmic in $n$?

\paragraph*{Our contribution.}
In this work we answer this question affirmatively by proving the following 
result.

\begin{theorem}[Main result, stated informally]\label{thm:main-informal}
 There is a data structure that for a dynamic undirected graph $G$ updated by edge insertions and deletions, maintains whether $G$ contains a simple path on $k$ vertices with amortized update time $2^{\Oh(k^2)}$.
 The data structure assumes access to a dictionary on the edges of $G$.
\end{theorem}

Note that Theorem~\ref{thm:main-informal} is stated slightly informally, as we did not specify what we exactly mean by access to a dictionary on the edges of $G$.
This is a technical assumption that the edge set of $G$ can be indexed so that one can efficiently access a given edge and store some record associated with it.
A simple implementation of such a dictionary would be an adjacency matrix; then each dictionary operation can be carried out in constant time.
Of course the drawback is the quadratic initialization time and space complexity, but there are also more efficient possibilities:
for instance dynamic perfect hashing~\cite{dynamicHashing} would give linear space complexity and initialization time while offering dictionary operations with amortized expected $\Oh(1)$ time.
We discuss dictionaries in Section~\ref{sec:kpath}; the formal statement of Theorem~\ref{thm:main-informal}, given as Theorem~\ref{thm:main-formal}, can be found there as well.

\paragraph*{Our techniques.}
Instead of relying on color-coding, our idea is to resort to the earlier decomposition approach of Bodlaender~\cite{Bodlaender93}.
In modern terms, this approach can be explained as follows.
An {\em{elimination forest}} of a graph $G$ is a rooted forest $F$ on the same vertex set as $G$ where for every edge $uv$ of $G$, either $u$ is an ancestor of $v$ or vice versa.
The observation is that every DFS forest of a graph is an elimination forest.
Hence, if by applying a DFS we obtain an elimination forest $F$ whose depth is at least $k$, then we immediately see a $k$-path in the graph. 
Otherwise, we can employ a standard dynamic programming procedure on this forest to decide whether $G$ contains a $k$-path.

This reasoning shows an important connection between the $k$-path problem and the notion of the {\em{treedepth}} of a graph, which is the smallest possible depth of an elimination forest.
Namely, if $G$ does not contain a $k$-path, then the treedepth of $G$ is smaller than $k$.
Contrapositively, if the treedepth of $G$ is larger than $k$, then $G$ certainly contains a $k$-path.
This suggests the following strategy for the dynamic $k$-path problem: 
design a data structure that maintains a bounded-depth elimination forest of a dynamic graph, together with tables of a suitable dynamic programming algorithm for $k$-path.

This problem ---maintaining an elimination forest of a bounded treedepth graph dynamically modified by edge insertions and deletions --- has been considered by Dvo\v{r}\'ak et al.~\cite{DvorakKT14}.
They gave a data structure that maintains an elimination forest of optimum depth with update time $f(d)$, for some function $f$, provided that there is a promise that the treedepth never exceeds $d$.
Moreover, the data structure may maintain the answer to any fixed problem definable in {\em{Monadic Second Order logic}} $\MSO_2$ within the same update time.

Since containing a $k$-path can be expressed using an $\MSO_2$ sentence of size bounded by a function of $k$, all of this combined gives a data structure for the dynamic $k$-path problem with update time $f(k)$,
however working {\em{only}} under the following assumption: the treedepth of the graph in question always stays lower than $k$. Note that if this invariant ceases to hold, then we know for sure that a $k$-path exists, but 
the data structure should also handle a situation when the treedepth fluctuates above and below $k$.
We show that the promise can indeed be lifted using a simple technique of 
postponing invariant-breaking insertions in an auxiliary queue, which was used 
by Eppstein et al.~\cite{EppsteinGIS96} in the context of planarity testing.
This comes at the cost of introducing amortization. 
Also, this is the only place where we actually use the assumption that we are given access to a dictionary on the edge set of the graph.
We remark that this idea can also be applied to two data structures given by Alman et al.~\cite{AlmanMW17} --- for the {\sc{Edge Clique Cover}} and {\sc{Point Line Cover}} problems --- 
to remove the assumption about being given a promise that the considered dynamic instance always contains a solution of bounded size.

All of this combined gives a data structure for the dynamic $k$-path problem with amortized update time $f(k)$, for some function $f$.
Unfortunately, the obtained function $f$ depends on $k$ in a non-elementary way: it is a tower of height depending on $k$.
This is not only caused by encoding the $k$-path problem in $\MSO_2$, which could be avoided by hand-crafting an explicit dynamic programming procedure.
The more serious issue is that the implementation of the data structure of Dvo\v{r}\'ak et al.~\cite{DvorakKT14} actually uses answers to some quite complicated $\MSO_2$ queries in order to perform updates in the maintained elimination forest. 
Hence, the non-elementary update time is needed also for maintaining the forest itself.

Now, our approach can be summarized as follows. We present a new data structure for the problem considered by Dvo\v{r}\'ak et al.~\cite{DvorakKT14} that offers an improved update time of $2^{\Oh(d^2)}$.
This data structure can be combined with the standard dynamic programming approach to $k$-path to give a data structure for the $k$-path problem in a dynamic graph of treedepth smaller than $k$ with update time $2^{\Oh(k^2)}$.
Combining this with the technique of postponing insertions gives our main result, Theorem~\ref{thm:main-informal}.

The bulk of our work is devoted to the new data structure for maintaining an optimal elimination forest of a dynamic graph of bounded treedepth. 
Admittedly, our approach is heavily inspired by the general strategy of Dvo\v{r}\'ak et al.~\cite{DvorakKT14}, hence let us provide a comprehensive comparison.

\paragraph*{Comparison with Dvo\v{r}\'ak et al.~\cite{DvorakKT14}.}
Let $F$ be an elimination forest of a graph $G$. 
With any vertex $u\in V(G)$ we can associate a graph $G_u$ defined as the subgraph of $G$ induced by all the ancestors and descendants of $u$ in $F$.
The idea is to associate with each vertex $u$ the {\em{type}} of $G_u$, which is a piece of information that concisely describes all the properties of $G_u$ needed both for the task of computing the treedepth, 
and for verifying the $\MSO_2$-expressible property $\varphi$ we are interested in. 
In the work of Dvo\v{r}\'ak et al.~\cite{DvorakKT14}, this type is the $\MSO_2$ type of $G_u$ of sufficiently high quantifier rank $q$, depending on both $d$ and $\varphi$. We note that in~\cite{DvorakKT14}, 
this is presented somewhat differently. Namely, the type of $G_u$ is maintained implicitly by storing a bounded-size {\em{$S$-code}}: a representantive subgraph of $G_u$, obtained by trimming superfluous subtrees in $F$.

Now, basic compositionality and idempotence properties of $\MSO_2$ imply that in order to compute the type of $G_u$, it suffices to know the multiset of types of graphs $G_v$ for all children $v$ of $u$ in $F$.
Moreover, there is a threshold $\tau$ depending on $d$ and $\varphi$ such that within this multiset, each type appearing more than $\tau$ times can be treated as if it appeared exactly $\tau$ times.
Thus, for any vertex $u$ one can compute the type of $G_u$ from the types associated with the children in constant time, even though the number of children is unbounded. 
This allows efficient recomputation of the types upon modifications of the forest $F$.

The implementation of updates works roughly as follows. Suppose $F$ is a tree for simplicity. First, one finds a {\em{candidate new root}}: a vertex that may be the new root of an optimal elimination tree after the update. 
Now comes the main trick: being a candidate root can be expressed by a (quite complicated) $\MSO_2$ formula of quantifier rank $d$, 
hence we can use the types stored in $F$ before the update to locate a candidate root.
Once the new root is located, we iteratively move the new root up the tree. During this process we need to fix a bounded number of subtrees using a fairly convoluted recursion scheme.

Thus, the aspect that contributes the most to the time complexity is the number of types that the data structure needs to keep track of.
In~\cite{DvorakKT14}, Dvo\v{r}\'ak et al. used $\MSO_2$ types of a sufficiently high quantifier rank, whose number is bounded by a non-elementary function of $d$ and $\varphi$.
In our data structure, we are much more frugal in this aspect: we show that it is enough to classify each vertex $u$ according to (1) the treedepth of the subraph induced by the descendants of $u$, including $u$; 
and (2) the set of ancestors of $u$ that are adjacent to $u$ or any of its descendants. This gives only $d\cdot 2^d$ different types. 
Moreover, we perform the update in a different way than Dvo\v{r}\'ak et al.: to construct an elimination forest $F'$ of the updated graph, 
we extract a {\em{core}} $K\subseteq V(G)$ of size $d^{\Oh(d)}$ that contains both endpoints of the updated edge,
compute an optimum elimination forest $F^K$ of $G[K]$ using the static algorithm of Reidl et al.~\cite{ReidlRVS14} in time $2^{\Oh(d^2)}$, and construct $F'$ by re-attaching parts of $F$ lying outside of $K$ to $F^K$.
While this method is conceptually simpler than the approach used in~\cite{DvorakKT14}, justifying the correctness requires a quite deep and technical dive into the combinatorics of treedepth and of elimination forests.
We remark that the construction of the core is analogous to the construction of the $S$-codes in~\cite{DvorakKT14}, but is done more carefully so that the size of the core is much smaller.

\paragraph*{Obstructions for treedepth.}
We observe that our combinatorial analysis leading to the construction of a core of size $d^{\Oh(d)}$ can also be  used to give improved bounds on the sizes of minimal obstructions for having treedepth $d$ with respect 
to the induced subgraph order. Precisely, we say that a graph $G$ is a {\em{minimal obstruction for treedepth $d$}} if its treedepth is larger than $d$, but every proper induced subgraph of $G$ already has treedepth at most $d$.
Note that every graph of treedepth larger than $d$ contains some minimal obstruction for treedepth $d$ as an induced subgraph, hence such obstructions are minimal ``witnesses'' for having large treedepth.
Dvo\v{r}\'ak et al.~\cite{DvorakGT12} proved that every minimal obstruction for treedepth $d$ has at most $2^{2^{d-1}}$ vertices, and they gave a construction of an obstruction with $2^d$ vertices.
They also hypothesized that in fact, every minimal obstruction for treedepth $d$ has at most $2^d$ vertices.
We get closer to this conjecture by showing an improved upper bound of $d^{\Oh(d)}$.

\paragraph*{Other related work.}
Dvo\v{r}\'ak and T\r{u}ma~\cite{DvorakT13} investigated the problem of counting occurrences (as subgraphs) of a fixed pattern graph $H$ in a dynamic graph $G$ that is assumed to be sparse 
(formally, always belongs to a fixed class of bounded expansion $\Cc$). They gave a data structure that maintains such a count with amortized update time $\Oh(\log^{c} n)$, where the constant $c$ 
depends both on $H$ and on the class $\Cc$. As classes of bounded treedepth have bounded expansion (see~\cite{NesetrilM12}), by taking $H$ to be a path on $k$ vertices we obtain
a data structure for the dynamic $k$-path problem in graphs of treedepth smaller than $k$ with amortized polylogarithmic update time, where the degree of the polylogarithm depends on $k$.
Note that this result is weaker than that provided by Alman et al.~\cite{AlmanMW17}, though it is obtained using very different tools.

Besides the works mentioned above~\cite{AlmanMW17,DvorakT13,DvorakKT14}, we are aware only of a handful of other papers investigating the concept of dynamic parameterized algorithms.
While the dynamic setting for parameterized vertex cover and other vertex-deletion problems was first considered by Iwata and Oka~\cite{IwataO14}, 
the main reference point here is the work of Alman et al.~\cite{AlmanMW17}, who performed a systematic study of a dozen of fundamental parameterized problems and gave a basic methodology for proving lower bounds.
More recent advances include dynamic kernels for hitting and packing problems in set systems with very low update times~\cite{BannachHRT19},
and work on monitoring timed automata in data streams~\cite{GrezMPPR20}. Also, Schmidt et al.~\cite{SchmidtSVZK20} investigated a combination of parameterization and the concept of $\mathsf{DynFO}$.
This setting is, however, somewhat different, as the main focus is on performing updates that can be described using simple logical formulas, and not necessarily executable efficiently in the classic sense.

\paragraph*{Organization.} In Section~\ref{sec:prelims} we set up notation and recall basic definitions and facts about elimination forests. 
In Section~\ref{sec:cores} we work out the combinatorics of cores in elimination forests, while in Section~\ref{sec:obstructions} we digress to obtain improved bounds on the sizes of minimal obstructions for treedepth $d$.
In Section~\ref{sec:data-structure} we design a data structure that
maintains an optimal elimination forest in a dynamic graph of bounded treedepth. In Section~\ref{sec:dp} we show how this data structure can be enriched for the purpose of maintaining the run of an auxiliary
dynamic program, and we show such a dynamic program for the $k$-path problem.
In Section~\ref{sec:kpath} we discuss the technique of postponed insertions and gather all the tools to prove the main result. 
We conclude in Section~\ref{sec:conclusions} by discussing open problems.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> pseudocodes.tex <==
\section{Pseudocodes}\label{sec:pseudocodes}








%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

